Separability and harmony in ecumenical systems

The quest of smoothly combining logics so that connectives from classical and intuitionistic logics can co-exist in peace has been a fascinating topic of research for decades now. In 2015, Dag Prawitz proposed a natural deduction system for an ecumenical first-order logic. We start this work by proposing a {\em pure} sequent calculus version for it, in the sense that connectives are introduced without the use of other connectives. For doing this, we extend sequents with an extra context, the stoup, and define the ecumenical notion of polarities. Finally, we smoothly extend these ideas for handling modalities, presenting pure labeled and nested systems for ecumenical modal logics.

==> rules.tex <==
%!TEX root = main-JLC.tex
% !TEX spellcheck = en-US

\begin{itemize}
\item {\bf Intuitionistic and neutral rules.} The rules for intuitionistic and neutral right rules are applied over formulas in the stoup. The left rules are the same as in $\LE$. As an example,
\[
\infer[{\iimp R}]{\Seq{\Gamma}
{A\iimp B}{\Delta}}{\Seq{\Gamma,A}{ B}{\Delta}}
\]
\[
\infer[{\iimp L_a}]{\Seq{\Gamma, A\iimp B}{
\Pi}{\Delta}}
{\Seq{\Gamma, A\iimp B}{ A}{\Delta} & \Seq{\Gamma , B} 
{\Pi}\Delta} 
\quad
\infer[{\iimp L_m}]{\Seq{\Gamma_1, \Gamma_2,A\iimp B}{
\Pi}{\Delta_1,\Delta_2}}
{\Seq{\Gamma_1, A\iimp B}{ A}{\Delta_1} & \Seq{\Gamma_2 , B} 
{\Pi}{\Delta_2}} 
\]
for additive and multiplicative versions, respectively.
\item {\bf Classical rules.} Since the classical connectives are equivalent to negated non-externally classical formulas, {\em focusing} over an externally classical formula necessarily erases the stoup, both on the right and on the left. For example,
since $A\cimp B\equiv \neg(A\wedge \neg B)$, the $\LE$ derivations
\[
\infer{\Gamma, \neg(A\wedge \neg B)\seq\Pi}{
\infer{\Gamma, \neg(A\wedge \neg B)\seq A\wedge \neg B}
{\deduce{\Gamma, \neg(A\wedge \neg B)\seq A}{} & \infer{\Gamma, \neg(A\wedge \neg B)\seq \neg B}{\Gamma, \neg(A\wedge \neg B), B\seq \cdot}}}\qquad
\infer{\Gamma\seq \neg(A\wedge \neg B)}
{\infer{\Gamma, A\wedge \neg B\seq\cdot}
{\Gamma, A, \neg B\seq\cdot}}
\]
justify the rules
\[
\infer[\cimp L_a]{\Seq{\Gamma, A \rightarrow_c B}{\Pi}{\Delta} }{\Seq{\Gamma, A \rightarrow_c B}{ A}{\Delta}&\Seq{\Gamma, B}{\cdot}{\Delta}}
\qquad
\infer[\cimp R]{\Seq{\Gamma} {\Pi}{A
\rightarrow_c B, \Delta}}{\Seq{\Gamma, A}{  \cdot}{B,\Delta}} 
\]
The rules for the multiplicative case and right rules on stoup are
\[
\infer[\cimp L_m]{\Seq{\Gamma_1,\Gamma_2, A \rightarrow_c B}{\cdot}{\Delta_1,\Delta_2} }{\Seq{\Gamma_1}{ A}{\Delta_1}&\Seq{\Gamma_2, B}{\cdot}{\Delta_2}}
\qquad
\infer[\cimp R]{\Seq{\Gamma} {A
\rightarrow_c B}{ \Delta}}{\Seq{\Gamma, A}{  \cdot}{B,\Delta}} 
\]
\item {\bf Negation.} Negation is particular. First of all, negated formulas are negative by default. But also because the negated formula $\neg A$ can be seen as $A\cimp \bot$ or $A\iimp \bot$. Hence the $\LE$ derivations
\[
\infer{\Gamma, \neg A\seq\Pi}
{\Gamma, \neg A\seq A}
\qquad 
\infer{\Gamma\seq \neg A}{\Gamma, A\seq \cdot}
\]
justify the rules
\[
\begin{array}{c@{\qquad}c}
\infer[{\neg L}]{\Seq{\Gamma,\neg A}{\Pi}{\Delta}
}{\Seq{\Gamma, \neg A}{  A}{\Delta}}
\qquad
\infer[{\neg R}]{\Seq{\Gamma} 
{\Pi}{\Delta,\neg A}}{\Seq{\Gamma,A}{  \cdot}{\Delta}}
\end{array}
\]
or, equivalently in the presence of $\W_i$
\[
\begin{array}{c@{\qquad}c}
\infer[{\neg L}]{\Seq{\Gamma,\neg A}{\cdot}{\Delta}
}{\Seq{\Gamma, \neg A}{ A}{\Delta}}
\qquad
\infer[{\neg R}]{\Seq{\Gamma} 
{\neg A}{\Delta}}{\Seq{\Gamma,A}{  \cdot}{\Delta}}
\end{array}
\]

\end{itemize}

%Observe that the propositional introduction rules form a conservative extension of the rules in $\LC$, with a more modern presentation of negative formulas being {\em stored}, with a dual behavior from the decide rule $\D$, which choses a right-positive formula to be worked on.

This determines positive/negative phases in derivations, and the dynamic of the rules for classical connectives in $\LCE$ is as follows. Negative formulas in the classical contexts are eagerly decomposed; if a positive formula in the right context  is chosen to be worked on, it is placed in the stoup $\Pi$, and is treated intuitionistically.

Figure~\ref{fig:LCE} brings the rules for the additive version of ecumenical pure systems with persistent stoup ($\LCE$).
%, while Figure~\ref{fig:LCEm} depicts the rules for  the multiplicative version of ecumenical pure systems with non-persistent stoup ($\LCEm$).
 
%Any mixture of these ideas may result into interesting proof systems.

\begin{figure}[htp]
{\sc Intuitionistic and neutral Rules}
\[
\begin{array}{c@{\qquad}c}
\infer[{\iimp L}]{\Seq{\Gamma, A\iimp B}{
\Pi}{\Delta}}
{\Seq{\Gamma, A\iimp B}{ A}{\Delta} & \Seq{\Gamma , B} 
{\Pi}\Delta} 
 &
\infer[{\iimp R}]{\Seq{\Gamma}
{A\iimp B}{\Delta}}{\Seq{\Gamma,A}{ B}{\Delta}}
\\[5pt]
\infer[{\vee_i L}]{\Seq{\Gamma, A \vee_i B}{ \Pi}{\Delta}
}{\deduce{\Seq{\Gamma, A}{ \Pi}{\Delta}}{} &\deduce{\Seq{\Gamma,B}{\Pi}{\Delta}}{}} 
& 
\infer[{\vee_i R_j}]{\Seq{\Gamma}{ A_1\vee_i A_2}{\Delta}}{\Seq{\Gamma}{ A_j}{\Delta}} 
\\[5pt]
\infer[\exists_i L]{\Seq{\Gamma, \exists_ix.A}{ \Pi}{\Delta}}{\Seq{\Gamma, A[y/x]}{ \Pi}{\Delta}}
&
\infer[\exists_i R]{\Seq{\Gamma}{ \exists_ix.A}{\Delta }}{\Seq{\Gamma}{ A[y/x]}{\Delta}}
\\[5pt]
\infer[{\wedge L}]{\Seq{\Gamma, A \wedge B}{ \Pi} {\Delta}}{\Seq{\Gamma,
A, B}{ \Pi}{\Delta}} 
&
\infer[{\wedge R}]{\Seq{\Gamma}
{A \wedge B}{\Delta}}{\deduce{\Seq{\Gamma} {A}{\Delta}}{} &\deduce{\Seq{\Gamma}{  B}{\Delta}}{}} 
\\[5pt]
\infer[\forall L]{\Seq{\Gamma,\forall x.A}{ \Pi}{\Delta}}{\Seq{\Gamma,\forall x.A,A[y/x]}{ \Pi}{\Delta}}
&
\infer[\forall R]{\Seq{\Gamma}{ \forall x.A}{\Delta}}{\Seq{\Gamma}{ A[y/x]}{\Delta}}
%\infer[{\bot L}]{\Gamma,\bot \seq \Delta}{}
%&
\end{array}
\]
{\sc Negation}
\[
\begin{array}{c@{\qquad}c}
\infer[{\neg L}]{\Seq{\Gamma,\neg A}{\Pi}{\Delta}
}{\Seq{\Gamma, \neg A}{  A}{\Delta}}
&
\infer[{\neg R}]{\Seq{\Gamma} 
{\Pi}{\Delta,\neg A}}{\Seq{\Gamma,A}{  \cdot}{\Delta}}
\end{array}
\]
{\sc Classical Rules}
\[
\begin{array}{c@{\qquad}c}
\infer[\cimp L]{\Seq{\Gamma, A \rightarrow_c B}{\Pi}{\Delta} }{\Seq{\Gamma, A \rightarrow_c B}{ A}{\Delta}&\Seq{\Gamma, B}{\cdot}{\Delta}}
&
\infer[\cimp R]{\Seq{\Gamma} {\Pi}{A
\rightarrow_c B, \Delta}}{\Seq{\Gamma, A}{  \cdot}{B,\Delta}} 
\\[5pt]
\infer[\vee_cL]{\Seq{\Gamma,  A \vee_c B}{\Pi}{\Delta}}{\Seq{\Gamma,A}{ \cdot}{\Delta} & \Seq{\Gamma,B}{ \cdot}{\Delta}} 
&
\infer[\vee_cR]{\Seq{\Gamma}{ \Pi}{ A \vee_c B,\Delta}}{\Seq{\Gamma}{ \cdot}{A,B,\Delta}}
\\[5pt]
\infer[\exists_c L]{\Seq{\Gamma ,\exists_cx.A}{ \Pi}{\Delta}}{\Seq{\Gamma,  A[y/x]}{ \cdot}{\Delta}}
&
\infer[\exists_c R]{\Seq{\Gamma}{ \Pi}{\exists_cx.A,\Delta}}{\Seq{\Gamma}{\cdot}{A[y/x],\exists_cx.A,\Delta}}
\\[5pt]
\infer[L_c]{\Seq{\Gamma, p_c}{\Pi}{\Delta}}{\Seq{\Gamma,p_i}{ \cdot}{\Delta}}
&
\infer[R_c]{\Seq{\Gamma}{ \Pi}{p_c,\Delta}}{\Seq{\Gamma}{ \cdot}{p_i,\Delta}} 
\end{array}
\]
{\sc Decision and Structural Rules}
\[
\begin{array}{c@{\qquad}c@{\qquad}c}
%\infer[{\W}]{\Gamma \seq I;\Delta}{\Gamma \seq \cdot;\Delta}
%&
\infer[\init]{\Seq{\Gamma,p_i}{ p_i}{\Delta}}{} 
&
\infer[\D]{\Seq{\Gamma}{ \cdot}{P,\Delta}}{\Seq{\Gamma}{ P}{P,\Delta}} 
&
\infer[\store]{\Seq{\Gamma}{ N}{\Delta}}{\Seq{\Gamma}{ \cdot}{N,\Delta}} 
\end{array}
\]
{\sc Cut Rules}
\[
\begin{array}{c@{\qquad}c}
\infer[P-\cut]{\Seq{\Gamma}{ \Pi}{\Delta}}{\Seq{\Gamma}{ P}{\Delta} & \Seq{P,\Gamma}{ \Pi}{\Delta}} 
&
\infer[N-\cut]{\Seq{\Gamma}{ \Pi}{\Delta}}{\Seq{\Gamma}{ \Pi}{\Delta, N} & \Seq{N,\Gamma}{ \cdot}{\Delta}} 
\end{array}
\]
\caption{Ecumenical pure system $\LCE$. In rules 
$\forall R$, $\exists_c L$ and $\exists_i L$, $y$ is fresh. $N$ is negative and $P$ is positive. $p$ is atomic.}\label{fig:LCE}
\end{figure}


%\begin{figure}[htp]
%{\sc Intuitionistic and neutral Rules}
%\[
%\begin{array}{c@{\qquad}c}
%\infer[{\iimp L}]{\Seq{\Gamma_1,\Gamma_2, A\iimp B}{
%\Pi}{\Delta_1,\Delta_2}}
%{\Seq{\Gamma_1, A\iimp B}{ A}{\Delta_1} & \Seq{\Gamma_2 , B} 
%{\Pi}{\Delta_2}} 
% &
%\infer[{\iimp R}]{\Seq{\Gamma}
%{A\iimp B}{\Delta}}{\Seq{\Gamma,A}{ B}{\Delta}}
%\\[5pt]
%\infer[{\vee_i L}]{\Seq{\Gamma_1,\Gamma_2, A \vee_i B}{ \Pi}{\Delta_1,\Delta_2}
%}{\deduce{\Seq{\Gamma_1, A}{ \Pi}{\Delta_1}}{} &\deduce{\Seq{\Gamma_2,B}{\Pi}{\Delta_2}}{}} 
%& 
%\infer[{\vee_i R_j}]{\Seq{\Gamma}{ A_1\vee_i A_2}{\Delta}}{\Seq{\Gamma}{ A_j}{\Delta}} 
%\\[5pt]
%\infer[\exists_i L]{\Seq{\Gamma, \exists_ix.A}{ \Pi}{\Delta}}{\Seq{\Gamma, A[y/x]}{ \Pi}{\Delta}}
%&
%\infer[\exists_i R]{\Seq{\Gamma}{ \exists_ix.A}{\Delta }}{\Seq{\Gamma}{ A[y/x]}{\Delta}}
%\\[5pt]
%\infer[{\wedge L}]{\Seq{\Gamma, A \wedge B}{ \Pi} {\Delta}}{\Seq{\Gamma,
%A, B}{ \Pi}{\Delta}} 
%&
%\infer[{\wedge R}]{\Seq{\Gamma_1,\Gamma_2}
%{A \wedge B}{\Delta_1,\Delta_2}}{\deduce{\Seq{\Gamma_1} {A}{\Delta_1}}{} &\deduce{\Seq{\Gamma_2}{  B}{\Delta_2}}{}} 
%\\[5pt]
%\infer[\forall L]{\Seq{\Gamma,\forall x.A}{ \Pi}{\Delta}}{\Seq{\Gamma,\forall x.A,A[y/x]}{ \Pi}{\Delta}}
%&
%\infer[\forall R]{\Seq{\Gamma}{ \forall x.A}{\Delta}}{\Seq{\Gamma}{ A[y/x]}{\Delta}}
%%\infer[{\bot L}]{\Gamma,\bot \seq \Delta}{}
%%&
%\end{array}
%\]
%{\sc Negation}
%\[
%\begin{array}{c@{\qquad}c}
%\infer[{\neg L}]{\Seq{\Gamma,\neg A}{\cdot}{\Delta}
%}{\Seq{\Gamma, \neg A}{  A}{\Delta}}
%&
%\infer[{\neg R}]{\Seq{\Gamma} 
%{\neg A}{\Delta}}{\Seq{\Gamma,A}{  \cdot}{\Delta}}
%\end{array}
%\]
%{\sc Classical Rules}
%\[
%\begin{array}{c@{\qquad}c}
%\infer[\cimp L]{\Seq{\Gamma_1,\Gamma_2, A \rightarrow_c B}{\cdot}{\Delta_1,\Delta_2} }{\Seq{\Gamma_1, A \rightarrow_c B}{ A}{\Delta_1}&\Seq{\Gamma_2, B}{\cdot}{\Delta_2}}
%&
%\infer[\cimp R]{\Seq{\Gamma} {A
%\rightarrow_c B}{ \Delta}}{\Seq{\Gamma, A}{  \cdot}{B,\Delta}} 
%\\[5pt]
%\infer[\vee_cL]{\Seq{\Gamma_1,\Gamma_2,  A \vee_c B}{\cdot}{\Delta_1,\Delta_2}}{\Seq{\Gamma_1,A}{ \cdot}{\Delta_1} & \Seq{\Gamma_2,B}{ \cdot}{\Delta_2}} 
%&
%\infer[\vee_cR]{\Seq{\Gamma}{A \vee_c B}{ \Delta}}{\Seq{\Gamma}{ \cdot}{A,B,\Delta}}
%\\[5pt]
%\infer[\exists_c L]{\Seq{\Gamma ,\exists_cx.A}{ \Pi}{\Delta}}{\Seq{\Gamma,  A[y/x]}{ \cdot}{\Delta}}
%&
%\infer[\exists_c R]{\Seq{\Gamma}{\exists_cx.A}{\Delta}}{\Seq{\Gamma}{\cdot}{A[y/x],\exists_cx.A,\Delta}}
%\\[5pt]
%\infer[L_c]{\Seq{\Gamma, p_c}{\cdot}{\Delta}}{\Seq{\Gamma,p_i}{ \cdot}{\Delta}}
%&
%\infer[R_c]{\Seq{\Gamma}{p_c}{\Delta}}{\Seq{\Gamma}{ \cdot}{p_i,\Delta}} 
%\end{array}
%\]
%{\sc Decision and Structural Rules}
%\[
%\begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c}
%\infer[\W L]{A,\Gamma \Rightarrow \Delta ; \Pi}{\Gamma \Rightarrow \Delta ; \Pi}
%&
%\infer[\W_{c} R]{\Gamma \Rightarrow \Delta , A ; \Pi}{\Gamma \Rightarrow \Delta ; \Pi }
%&
%\infer[\W_{i} R]{\Gamma \Rightarrow \Delta ; A}{\Gamma \Rightarrow \Delta ; \cdot }
%\\[5pt]
%\infer[\C L]{A, \Gamma \Rightarrow C}{A, A, \Gamma \Rightarrow C}
%&
%\infer[\C R]{\Gamma \Rightarrow \Delta , A ; \Pi}{\Gamma \Rightarrow \Delta , A, A ; \Pi }
%&
%\infer[\D]{\Seq{\Gamma}{ \cdot}{\Delta,A}}{\Seq{\Gamma}{ A}{\Delta}} 
%\\[5pt]
%&\infer[\init]{\Seq{\Gamma,p_i}{ p_i}{\Delta}}{} 
%\end{array}
%\]
%{\sc Cut Rules}
%\[
%\begin{array}{c@{\qquad}c}
%\infer[i-\cut]{\Seq{\Gamma_1,\Gamma_2}{ \Pi}{\Delta_1,\Delta_2}}{\Seq{\Gamma_1}{ A}{\Delta_1} & \Seq{A,\Gamma_2}{ \Pi}{\Delta_2}} 
%&
%\infer[c-\cut]{\Seq{\Gamma_1,\Gamma_2}{ \Pi}{\Delta_1,\Delta_2}}{\Seq{\Gamma_1}{ \Pi}{\Delta_1, A} & \Seq{A,\Gamma_2}{ \cdot}{\Delta_2}} 
%\end{array}
%\]
%\caption{Ecumenical pure system $\LCEm$. In rules 
%$\forall R$, $\exists_c L$ and $\exists_i L$,  $y$ is fresh. $p$ is atomic.}\label{fig:LCEm}
%\end{figure}
%

